Smaller, Weaker, Yet Better: Training LLM Reasoners via Compute-Optimal Sampling

Training on high-quality synthetic data from strong language models (LMs) is a common strategy to improve the reasoning performance of LMs. In this work, we revisit whether this strategy is compute-optimal under a fixed inference budget (e.g., FLOPs). To do so, we investigate the trade-offs between generating synthetic data using a stronger but more expensive (SE) model versus a weaker but cheaper (WC) model. We evaluate the generated data across three key metrics: coverage, diversity, and false positive rate, and show that the data from WC models may have higher coverage and diversity, but also exhibit higher false positive rates. We then finetune LMs on data from SE and WC models in different settings: knowledge distillation, self-improvement, and a novel weak-to-strong improvement setup where a weaker LM teaches reasoning to a stronger LM. Our findings reveal that models finetuned on WC-generated data consistently outperform those trained on SE-generated data across multiple benchmarks and multiple choices of WC and SE models. These results challenge the prevailing practice of relying on SE models for synthetic data generation, suggesting that WC may be the compute-optimal approach for training advanced LM reasoners.

==> sections/sft_setup.tex <==
\section{Supervised Finetuning Setups}
\label{sec:sft_paradigms}

To evaluate the utility of the synthetic data, we train strong reasoners under three supervised finetuning setups. In all three setups, the finetune a model in synthetic data generated from the WC and SE models. The difference is in the model that is being finetuned. In the first setup, we finetune a separate (student) LM from the WC and SE models; we refer to this setup as \textit{Student-LM finetuning}. In the second setup, we finetune the WC model; we refer to this setup as \textit{WC-LM finetuning}. And in the third setup, we finetune the SE model; we refer to this setup as \textit{SE-LM finetuning}. These three setups give rise to diverse supervised finetuning paradigms from the literature as described below. 

\textbf{Knowledge Distillation:} corresponds to training a student LM on the synthetic data sampled from a strong and large LM. In our first setup, we finetune a smaller model based on the data from a WC and SE model separately. Both these setups correspond to sequential knowledge distillation \cite{}. So our first setup compares sequential knowledge distillation from a WC model vs a SE model.

\textbf{Self-Improvement:} corresponds to training a model on samples generated from itself. In our second setup, training the WC model on its own data corresponds to self-improvement whereas training WC on the data from SE corresponds to sequential knowledge distillation. So our second setup compares self-improvement from WC data vs knowledge distillation from SE data.
\textbf{Weak-to-Strong Improvement:}
We introduce a new paradigm, Weak-to-Strong Improvement (W2S-I), which focuses on \textit{enhancing} the reasoning capabilities of a strong model using samples generated by a weaker model. In our third setup, training SE on data from WC corresponds to W2S-I and training SE on data from SE corresponds to self-improvement. So our third setup compares W2S-I vs self-improvement.
Note that W2S-I is related to prior work \citep{burns2023weak} which introduced the concept of training strong models using data generated by weaker models. But in prior work, the specific aim is to recover the full capabilities of the strong model from weaker data, whereas we aim to enhance the strong model capabilities further. 
A summary of the three setups and the finetuning paradigms that each case corresponds to can be found in Table~\ref{tab:sft_setup_summary}.
